Simulating the inflationary Universe: from single-field to the axion-U(1) model

We present a nonlinear study of the inflationary epoch based on numerical lattice simulations. Lattice simulations are a well-known tool in primordial cosmology, and they have been extensively used to study the reheating epoch after inflation. We generalize this known machinery to the inflationary epoch. Being this the first simulation of the inflationary epoch much before the end of inflation, the first part of the thesis focuses on the minimal single-field model of inflation. We discuss the conceptual and technical ingredients needed to simulate inflation on a lattice. The simulation is used to reproduce the nearly scale-invariant spectrum of scalar perturbations, as well as the oscillations in the power spectrum caused by a step in the potential. In the second part, we focus on the more complicated axion-U(1) model of inflation and present the first lattice simulation of this model during the deep inflationary epoch. We use the simulation to discover new properties of primordial scalar perturbations from this model. In the linear regime of the theory, we find high-order non-Gaussianity (beyond trispectrum) to be key to describing the statistical properties of scalar perturbations. Conversely, we find perturbations to be nearly Gaussian in the nonlinear regime of the theory. This relaxes existing constraints from the overproduction of primordial black holes, allowing for a gravitational waves signal in the observable range of upcoming experiments such as LISA. Our results show that lattice simulations can be a powerful tool to study the inflationary epoch and its observational signatures.

==> Acknowledgement.tex <==
\chapter{Acknowledgements}

I would like to thank Ralf Bender for hosting me in his research group since the time of my Master's thesis and throughout my PhD studies. There must be a parallel reality somewhere (or is it ours?), of which the University Observatory is the heaven of...
I would also like to thank Stella Seitz and Daniel Gruen for their mentoring, support, useful discussions, and for keeping my spirit while navigating the perilous world of an international scientific collaboration.

Throughout the my time in the PhD I received a great amount of insight and joy from discussions with my friends and colleagues for which I am immensely grateful. Especially, I would like to mention discussions with Oliver Friedrich, Ben Hoyle and Ramona Augustin which helped me brighten my day in times when research seemed to hit a dead end.
Finally I would like to thank my parents, my family and my friends for supporting me throughout my studies.





==> newcommands.tex <==
\newcommand{\addgals}{\textsc{addgals}}


\newcommand{\wtg}{WtG}
\newcommand{\clash}{CLASH}
\newcommand{\cccp}{CCCP}
\newcommand{\locuss}{LoCuSS}

\newcommand{\simname}{\texttt{FOX}}
\newcommand{\rockstar}{{\tt Rockstar}}
\newcommand{\mangle}{\texttt{mangle}}

\newcommand{\gmag}{$g$}
\newcommand{\rmag}{$r$}
\newcommand{\imag}{$i$}
\newcommand{\zmag}{$z$}
\newcommand{\griz}{$g,r,i,z$}
\newcommand{\umg}{$u-g$}
\newcommand{\gmr}{$g-r$}
\newcommand{\rmi}{$r-i$}
\newcommand{\imz}{$i-z$}

\newcommand{\psfmag}{\texttt{psfmag}}
\newcommand{\modelmag}{\texttt{modelmag}}
\newcommand{\cmodelmag}{\texttt{cmodelmag}}

\newcommand{\radec}{$\alpha,\delta$}

\newcommand{\devauc}{De Vaucouleurs'}

\newcommand{\gammat}{\mbox{$\gamma^{\intercal}$}}

% peter's versions
\newcommand{\pzs}{\mbox{$p_\mathrm{phot}(z_{\mathrm{s},i})$ }}
\newcommand{\zsi}{\mbox{$z_{\mathrm{s},i}$}}
\newcommand{\zlj}{\mbox{$z_{\mathrm{l},j}$}}
\newcommand{\etan}{\mbox{$e^{\intercal}$}}
\newcommand{\etanij}{\mbox{$e^{\intercal}_{j,i}$}}

% erin's versions
%\newcommand{\pzs}{\mbox{$p(z_{\mathrm{s},i})$ }}
%\newcommand{\pzs}{\mbox{$p(z^i_{\mathrm{s}})$ }}
%\newcommand{\zsi}{\mbox{$z^i_\mathrm{s}$}}
%\newcommand{\zlj}{\mbox{$z^i_\mathrm{l}$}}
%\newcommand{\etani}{\mbox{$e^i_\mathrm{t}$}}

\newcommand{\gammacross}{$\gamma_\times$}
\newcommand{\deltasig}{$\Delta \Sigma$}
\newcommand{\dsig}{$\Delta\Sigma$}
\newcommand{\dsigr}{$\Delta\Sigma(R)$}
\newcommand{\dsigmis}{$\Delta\Sigma_{\mathrm{mis}}$}
\newcommand{\deltaplus}{$\Delta \Sigma_+$}
\newcommand{\deltacross}{$\Delta \Sigma_\times$}
\newcommand{\deltarho}{$\Delta \rho$}
\newcommand{\movr}{$M(<r)$}
\newcommand{\sigmacrit}{$\Sigma_{\mathrm{crit}}$}
\newcommand{\scinv}{$\Sigma^{-1}_{\mathrm{crit}}$}
\newcommand{\hinv}{h^{-1}}


\newcommand{\photoz}{\mbox{photo-$z$}}
\newcommand{\photozs}{\mbox{photo-$z$s}}

\newcommand{\lenszmax}{0.8}
\newcommand{\lenszmin}{0.2}

\newcommand{\hrs}{$^{\mathrm h}$}
\newcommand{\minutes}{$^{\mathrm m}$}

\newcommand{\redmapper}{redMaPPer}
\newcommand{\redmagic}{redMaGiC}
\newcommand{\rmversion}{6.3.3}
\newcommand{\ngmix}{\textsc{ngmix}\ }

\newcommand{\annz}{\textsc{annz2}}
\newcommand{\skynet}{\textsc{skynet}}
\newcommand{\tpz}{\textsc{tpz}}
\newcommand{\bpz}{\textsc{bpz}}
\newcommand{\balrog}{\textsc{Balrog}}
\newcommand{\cosmosis}{\textsc{CosmoSIS}}

\newcommand{\neffngmix}{5.7}
\newcommand{\ngmixlowzbiasneg}{$-0.04$}
\newcommand{\recommendedprior}{0.05}
\newcommand{\njack}{40}
\newcommand{\shapenoise}{0.22}
\newcommand{\rmax}{30}
\newcommand{\imshape}{{\textsc{im3shape}}}
\newcommand{\snr}{S/N}
\newcommand{\metacal}{\textsc{metacalibration}}

\newcommand{\msun}{\mathrm{M}_{\odot}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}


\newcommand{\edens}{$e_q$}
\newcommand{\lfsens}{\mbox{\boldmath $s$}}

\newcommand\avg[1]{\langle #1 \rangle}
\newcommand{\Scrit}{\Sigma_{\rm crit}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\hMpc}{h^{-1}\ \Mpc}

\newcommand{\fcl}{f_\mathrm{cl}}

\newcommand{\Mobs}{M_{\rm obs}}
\newcommand{\Mtrue}{M_{\rm true}}
\newcommand{\Var}{{\rm Var}}

\newcommand{\Rmis}{R_{\rm mis}}
\newcommand{\fmis}{f_{\rm mis}}
\newcommand{\cmis}{c_{\rm mis}}

\newcommand{\Am}{A_{\rm m}}

\newcommand{\lkhd}{{\cal L}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calC}{{\cal C}}

